Flow Priors for Linear Inverse Problems via Iterative Corrupted Trajectory Matching

Generative models based on flow matching have attracted significant attention for their simplicity and superior performance in high-resolution image synthesis. By leveraging the instantaneous change-of-variables formula, one can directly compute image likelihoods from a learned flow, making them enticing candidates as priors for downstream tasks such as inverse problems. In particular, a natural approach would be to incorporate such image probabilities in a maximum-a-posteriori (MAP) estimation problem. A major obstacle, however, lies in the slow computation of the log-likelihood, as it requires backpropagating through an ODE solver, which can be prohibitively slow for high-dimensional problems. In this work, we propose an iterative algorithm to approximate the MAP estimator efficiently to solve a variety of linear inverse problems. Our algorithm is mathematically justified by the observation that the MAP objective can be approximated by a sum of $N$ ``local MAP'' objectives, where $N$ is the number of function evaluations. By leveraging Tweedie's formula, we show that we can perform gradient steps to sequentially optimize these objectives. We validate our approach for various linear inverse problems, such as super-resolution, deblurring, inpainting, and compressed sensing, and demonstrate that we can outperform other methods based on flow matching. Code is available at https://github.com/YasminZhang/ICTM.

==> RelatedWorks.tex <==
\section{Related Works}


\ol{Good idea! I think in terms of subjects, we can talk about diffusion models for inverse problems, flow-based models, other learning-based algorithms that use an MAP approach}

\paragraph{Inverse Problems} It is an ill-posed problem. don't have lots of paired data: 1) unavaialbe 2) too expensive, cause trouble to patients.  
No paired data, only the measurements $y$ are observed. The inverse problems includes medical Medical, blackhole, etc... 
As more powerful pretrained generative models are at hand, our paper aims to unlock the potential of flow-based generative models to solve inverse problems. 

 


\paragraph{Flow-based Models} Neural ODE \cite{neuralODE} transform the evolution of intermediate layers as an ODE process. \cite{liu2022flow, liu2022c-rectified} use the optimal transport perspective. \cite{lipman2022flow} flow matching perspective displacement transport between two Gaussian distributions. Both perspectives rethink the role of diffusion in current generative models. Guided flow models \cite{zheng2023guidedflow} \cite{hu2024adaflow} decision makers also show superior performance on many tasks. Instaflow \cite{liu2023instaflow} and Stable diffusion 3 \cite{esser2024scaling} large scale text-to-image datasets.


\paragraph{MAP for Inverse Problems} DPS \cite{chung2023diffusion}  aims to do posterior sampling in the reverse process of the diffusion. 
Without the explicit formulation of the gradient of probability at timestep $t$, 
\cite{pokle2023training} solve the linear inverse problems via flows. 
